A democratic Cosmos?

Despite the success of our best models in Theoretical Physics, especially concerning Cosmology and Particle Physics, we still face persistent challenges. Among them we have the cosmological singularity problem, understanding the late-time acceleration of the Universe, and comprehending the fundamental nature of time. We believe relevant new insights to tackle each of these issues may be found in the Philosophy of Cosmology. We elaborate on three philosophical principles that shall guide us on how to improve our current theories. They are the Copernican Principle for Scales, the Cosmological Heterarchical Principle and the Cosmological Principle of Irreversibility. Following these principles, and using some of our current physical theories as a proxy to implement them, we consider a new assessment of each of these challenges, and show how they may be either explained away, hinting towards new physics, or summarized in a new philosophical principle.

==> sections/lambda+.tex <==
\subsection{[Things we haven't yet included in the IR section]}

\begin{itemize}

    \item Perhaps DE and DM arise from a common origin, such as in the superfluid DM model [citation needed] \Gui{(They don't actually relate both scales, as far as I know. The only thing DM superfluid models can do it to relate the DM and DE phenomena into a common origin, but not really accounting for such coincidence.)}

    \item de Sitter symmetry in higher dimensions? Maybe Lorentz symmetry and scale invariance arise from a spontaneous symmetry breaking of such a (de Sitter) group in two different ways?
    
    \item The Baryonic Tully Fisher Relationship (we can use fig. 3 from here: https://arxiv.org/pdf/1112.3960.pdf) correlates the baryonic mass $M_b$ contained within the galaxy to the asymptotic circular velocity $v_c$, 
    \begin{equation}
        M_b \sim v_c^4.
    \end{equation}
    In the context of MOdified Newtonian Mechanics (MOND, see reference), the proportionality constant is fixed to be, 
    \begin{equation}
        M_b = \frac{v_c^4}{G a_0} \label{eq:BTFR},
    \end{equation}
    where $a_0$ defines a critical acceleration scale for which the best-fit value is of order of the current Hubble parameter, 
    \begin{equation}
        a_0 \simeq \frac{c}{6}H_0 \simeq 1.2\times 10^{-8} \text{cm/s$^2$}.
    \end{equation}
    The fact that $a_0$ is coincidental to $H_0$ is a mystery either in the context of SMC or MOND. We believe, however, it is a hint for the presence of a modification of deep infra-red regime of gravity.
    
    \item One way to contemplate that is rewriting \ref{eq:BTFR} as,
    \begin{equation}
    \frac{r_S}{r_\Lambda} = 12 \left( \frac{v_c}{c}\right)^4,
    \end{equation}
    where $r_S$ corresponds to the Schwarzschild radius of the galaxy and $r_\Lambda$ corresponds to the radius of the de Sitter horizon. While the RHS looks like a UV EFT expansion parameter, which increases as one increases momentum, the LHS looks like an IR coupling, since it increases as larger distances are allowed.
    
    \item https://arxiv.org/pdf/1610.08981.pdf 
    [The basic tenet of MOND is that dynamics become scale-invariant below a critical acceleration scale a0 (Milgrom 2009, https://arxiv.org/pdf/0810.4065.pdf): the equations of motion remain unchanged under the transformation (r, t) → (λr, λt).]
    
    \item Mond as evidence \Gui{(suggestion: maybe to write $\sqrt{UV \times IR} = MOND-scale$ as a pictoresque way of understanding why MOND is evidence, thus commenting on the coupling between Hubble radius and Schwarzschild radius). From Mcgaugh's paper: "The radial acceleration relation subsumes and generalizes several well-known dynamical properties of galaxies, like the Tully-Fisher and Faber-Jacson relations, the "baryon-halo" conspiracies, and Renzo's rule". }
    
    \item \Gui{suggestion: maybe we should talk about MOND-like dynamics, since we are not really advocating for MOND, but to something that reproduce MOND; we just use the term since it was the first attempt to fit the data that was being observed}
    
    \Gui{I've just seen this paper: https://arxiv.org/pdf/astro-ph/9303012.pdf where Milgrom, back in 1993, already conjectures that MOND must be an effective theory of some other theory living at the large - so we need to cite it for sure}
    
    \item \Yig{(Verlinde's theory of Emergent Gravity might also be worth mentioning somewhere.) \Gui{(We would need to check if his model accounts for the coincidence. However, his model is really ad hoc as far as I remember, and plunged with problems. Worth checking it anyhow.)}} \Yig{(The relevant paper is 1611.02269. In the equation (7.43), he relates the MOND acceleration scale $a_M$ to the de Sitter acceleration scale $a_0$ (defined in eq.~(1.2)) and postdicts the ratio as 1/6.)}
    
   \end{itemize}

==> sections/newdirections.tex <==

\begin{itemize}

    
    \item The second part of the project will dive more deeply into two pressing conceptual issues
    
    \begin{itemize}
        \item  (1) the epistemological significance of the crucial role now played by
simulations in linking cosmological theory with observations

        \item (2) the status of the large-scale structure of the universe in light of
suggestions from quantum gravity that characteristic features of general relativity, such as singularities, may not persist into future theories
    \end{itemize}
    
    \item  One of the striking things about the ongoing methodological debates in cosmology is that they rely on distinctions and criteria – science and pseudoscience; falsifiability – that philosophers of science have long argued never adequately captured successful scientific practice. Instead, most philosophers of science today accept some variety of belief-revision model of knowledge, according to which theories (or models) have more or less support, given the available evidence, but no evidence should be taken as straightforwardly confirmatory or falsifying. This picture of the relation between evidence and belief seems far better suited to the situation in cosmology than the one cosmologists appear to have inherited from a previous generation of physicists. And if accepted by cosmologists, it could radically restructure current disputes about the state of the field.
    
    \item \textbf{Central Questions:}
    \begin{itemize}
        \item Is it possible to discover and justify new fundamental laws in cosmology?
        
        \item Does cosmology require new rules for testing theories?
        
        \item What is the status of spacetime concepts in cosmology? (this we can definitely tackle directly in the context of T-duality)
        
     \end{itemize}
\end{itemize}

\section*{Important Points to Keep in Mind}

\begin{itemize}
      \item Smolin argues that a new strategy for quantum gravity is based on principles: 
    
    \begin{itemize}
        \item we should derive tests directly from principles if possible, as Einstein did with the equivalence principle for taling about the bending of light, for instance (we can associate this to MOND phenomenology, even though it would be posthoc for the time being)
        
        \item we should look for new domains of QG phenomena if this is really the theory we expect it to be (that's what we are doing here somehow)
        
        \item his full strategy is: 1) propose principles for QG; 2) show they suffice to derive GR; 3) derive experimental tests; 4) look for new regimes of QG; 5) employ models to connect principles to predictions 
        
        \end{itemize}
        
\end{itemize}

==> sections/standard_cosmology.tex <==
The SMC challenges our democratic tastes. When we look to some of its features, as for instance the idea that the whole background evolution of the universe for most of its existence can be parametrized by a single perfect fluid with an evolving equation of state, we are delighted by its simplicity. However, when we decompose further this fluid in its components and realize that some of them seem to have coincidentally the same power at our current time, which would account for a true manifestation of democracy in the Cosmos, we end up perplexed. 

Coincidence problem -> problem of scales 
cosmological constant problem -> $\Lambda$

the singularity problem 

\subsection{Is de Sitter a dictator?}

Of course, Willem de Sitter was not a dictator. This is just a cosmological joke, maybe of not so much cosmological laughter. In any case, when we look closely to the parable of the Universe, it seems that only for a short period of the time we have taken the power away from an almost-like de Sitter solution. When we say \emph{we have taken the power} that is actually more precisely than it seems at a first look, since we are after all made up of ordinary matter and our reign has been quite short. 
The SMC, at least for most of the community, also embeds the paradigm of inflation to the early universe. Inflation summons an accelerated expansion phase of the early Universe that explains why the Universe we live in seems to be so spatially flat, so large and how the fluctuations on the Cosmic Microwave Background (CMB) are almost scale-invariant, therefore also explaining how structures have been formed in our Universe. Most of the models for inflation rely in a quasi-de Sitter initial phase that smoothly shifts towards standard radiation decelerated expansion.

It feels somehow surprising that the current data once interpreted within the Standard Model demands the introduction of a dark component called dark energy. It has been observed in 1998 that our universe, given reasonable assumptions, seem to be expanding in an accelerated fashion. Since this phase has not started long ago and since we are still here and do observe matter (either baryonic or dark matter) to be still around, this expansion is also a quasi-de Sitter one. In fact, so far, the data is best fitted when we assumed that we are walking towards a pure de Sitter solution of the background, best accounted for the presence of a cosmological constant in Einstein Equations. 

Thus, if inflation has really happened and if the cosmological constant remains to be the best description of our late time cosmology, it does seem that the ruler of the background cosmology is (quasi)-de Sitter. Hence, it makes sense to feel perplexed that it is so coincidental that we live in a time where all the components contribute the same to the dynamics of the Cosmos, since that only implies we are already being overruled by the presence of DE. 

\footnote{Another misleading statement is to remain saying, even after General Relativity, that gravity is attractive. In General Relativity gravity is purely inertia encoded by the local geometry of spacetime, and that, surely, can have objects coming closer together or drifting apart from each other. A short way of replying to that statement is to say: de Sitter spacetime is gravitational!}
